A Picture is Worth More Than 77 Text Tokens: Evaluating CLIP-Style Models on Dense Captions

Curation methods for massive vision-language datasets trade off between dataset size and quality. However, even the highest quality of available curated captions are far too short to capture the rich visual detail in an image. To show the value of dense and highly-aligned image-text pairs, we collect the Densely Captioned Images (DCI) dataset, containing 7805 natural images human-annotated with mask-aligned descriptions averaging above 1000 words each. With precise and reliable captions associated with specific parts of an image, we can evaluate vision-language models' (VLMs) understanding of image content with a novel task that matches each caption with its corresponding subcrop. As current models are often limited to 77 text tokens, we also introduce a summarized version (sDCI) in which each caption length is limited. We show that modern techniques that make progress on standard benchmarks do not correspond with significant improvement on our sDCI based benchmark. Lastly, we finetune CLIP using sDCI and show significant improvements over the baseline despite a small training set. By releasing the first human annotated dense image captioning dataset, we hope to enable the development of new benchmarks or fine-tuning recipes for the next generation of VLMs to come.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%\newcommand{\florian}[1]{{\color{blue}[Florian: #1]}}

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


\def\tocite{{\color{red}[CITE]} }
\def\todo{{\color{red}[TODO]} }


\usepackage{graphicx}
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{collcell}
\usepackage{xifthen}
\usepackage{tikz}

\usepackage{xcolor}[table, dvipsnames] % enables the use of cellcolor make sure you have [table] option in the document class 
\usepackage{pgf} % for calculating the values for gradient
\usepackage{etoolbox}

